A Methodological Analysis of Empirical Studies in Quantum Software Testing

In quantum software engineering (QSE), quantum software testing (QST) has attracted increasing attention as quantum software systems grow in scale and complexity. Since QST evaluates quantum programs through execution under designed test inputs, empirical studies are widely used to assess the effectiveness of testing approaches. However, the design and reporting of empirical studies in QST remain highly diverse, and a shared methodological understanding has yet to emerge, making it difficult to interpret results and compare findings across studies. This paper presents a methodological analysis of empirical studies in QST through a systematic examination of 59 primary studies identified from a literature pool of size 384. We organize our analysis around ten research questions that cover key methodological dimensions of QST empirical studies, including objects under test, baseline comparison, testing setup, experimental configuration, and tool and artifact support. Through cross-study analysis along these dimensions, we characterize current empirical practices in QST, identify recurring limitations and inconsistencies, and highlight open methodological challenges. Based on our findings, we derive insights and recommendations to inform the design, execution, and reporting of future empirical studies in QST.

==> figures/generated/rq10_available_artifacts.tex <==

\begin{tabular}{c p{0.99\columnwidth}}
    \toprule[1pt]
    
    \multicolumn{2}{l}{\textbf{Software testing:}} \\
    \cite{\PaperOne} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/muskit}}, \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/5288917}} \\
    \cite{\PaperThree} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/quito}}, \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/5288665}} \\
    \cite{\PaperFive} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/qucat-tool}} \\
    \cite{\PaperThirteen} & \textit{GitHub}: {\footnotesize \url{https://github.com/ShahinHonarvar/QSharpCheck}} \\
    \cite{\PaperSeventeen} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/qusbt-tool}} \\
    \cite{\PaperTwenty} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/MutTG-paper}} \\
    \cite{\PaperTwentyOne} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/qusbt/}} \\
    \cite{\PaperTwentyFour} & \textit{GitHub}: {\footnotesize \url{https://github.com/LuisLlana/metamorphic_testing/}} \\
    \cite{\PaperTwentySeven} & \textit{GitHub}: {\footnotesize \url{https://github.com/biromiro/feup-gulbenkian-qc-mt}} \\
    \cite{\PaperThirtyThree} & \textit{Figshare}: {\footnotesize \url{https://figshare.com/articles/software/Delta_Debugging_for_Property-Based_Regression_Testing_of_Quantum_Programs/25075154?file=44241593}}, \textit{GitHub}: {\footnotesize \url{https://github.com/GabrielPontolillo/ddregression}} \\
    \cite{\PaperThirtySix} & \textit{GitHub}: {\footnotesize \url{https://github.com/am0x00/QuanTest}} \\
    \cite{\PaperThirtySeven} & \textit{GitHub}: {\footnotesize \url{https://github.com/cccorn/Q-ATPG}} \\
    \cite{\PaperThirtyEight} & \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/13370788}} \\
    \cite{\PaperThirtyNine} & \textit{GitHub}: {\footnotesize \url{https://github.com/AsmarMuqeet/QOPS}} \\
    \cite{\PaperFortyThree} & \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/11191215}} \\
    \cite{\PaperFortySix} & \textit{Zenodo}: {\footnotesize \url{https://doi.org/10.5281/zenodo.15462299}} \\
    \cite{\PaperFiftyNine} & \textit{Personal Website}: {\footnotesize \url{https://simula-complex.github.io/Quantum-Software-Engineering/ICST21.html}} \\
    \cite{\PaperSixty} & \textit{GitHub}: {\footnotesize \url{https://github.com/Simula-COMPLEX/qucat-paper}} \\
    \cite{\PaperSixtySeven} & \textit{GitHub}: {\footnotesize \url{https://github.com/WindFrank/QuantumDataAndProgram}} \\
    \cite{\PaperSeventy} & \textit{GitHub}: {\footnotesize \url{https://github.com/MgcosA/EvaluationCodeOfQuantumRelationChecking/}} \\
    \cite{\PaperSeventyFour} & \textit{GitHub}: {\footnotesize \url{https://github.com/danielfobooss/mutpy}} \\
    \cite{\PaperSeventyEight} & \textit{GitHub}: {\footnotesize \url{https://github.com/EnautMendi/Quantum-Circuit-Mutants-Empirical-Evaluation}} \\
    \cite{\PaperNinetyFour} & \textit{Figshare}: {\footnotesize \url{https://figshare.com/articles/software/QuCheck_with_QOIN/28772231}} \\
    \cite{\PaperOneHundredAndSix} & \textit{GitHub}: {\footnotesize \url{https://github.com/MgcosA/Code_of_Testing_Oracle_Quantum_Program_Article}} \\
    \cite{\PaperOneHundredAndThirteen} & \textit{GitHub}: {\footnotesize \url{https://github.com/sinugarc/QCRMut}} \\
    \cite{\PaperOneHundredAndFourteen} & \textit{GitHub}: {\footnotesize \url{https://github.com/csiro/QUT/tree/main}} \\
    \cite{\PaperOneHundredAndSixteen} & \textit{GitHub}: {\footnotesize \url{https://github.com/Ahmik-Virani/Differentiating-Quantum-Bug-From-Noise-Statistical-Approach}} \\
    \cite{\PaperOneHundredAndNineteen} & \textit{Figshare}: {\footnotesize \url{https://figshare.com/articles/software/QuCheck_A_Property-based_Testing_Framework_for_Quantum_Programs_in_Qiskit/27919539?file=53357996}} \\
    \cmidrule(lr){1-2}

    \multicolumn{2}{l}{\textbf{Runtime assertion:}} \\
    \cite{\PaperFortyOne} & \textit{OSF}: {\footnotesize \url{https://osf.io/k6ygp/overview}} \\
    \cite{\PaperFiftyFour} & \textit{GitHub}: {\footnotesize \url{https://github.com/munich-quantum-toolkit/debugger}} \\
    \cite{\PaperOneHundredAndFifteen} & \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/15708438}} \\
    \cite{\PaperOneHundredAndTwentyTwo} & \textit{GitHub}: {\footnotesize \url{https://github.com/revilooliver/Quantum-Circuits-for-Dynamic-Runtime-Assertions-in-Quantum-Computation}}, \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/3597507}} \\
    \cmidrule(lr){1-2}

    \multicolumn{2}{l}{\textbf{Program repair:}} \\
    \cite{\PaperFortyFour} & \textit{Zenodo}: {\footnotesize \url{https://zenodo.org/records/14288140}} \\
    \cmidrule(lr){1-2}

    \multicolumn{2}{l}{\textbf{Platforms: } \textit{GitHub} (24), \textit{Zenodo} (8), \textit{Figshare} (3), \textit{OSF} (1), \textit{Personal Website} (1)} \\
    \multicolumn{2}{l}{\textbf{Proportion of available artifacts}: 55.9\% (33/59)} \\
    \bottomrule[1pt]
\end{tabular}


==> figures/generated/rq10_available_program_sources.tex <==

\begin{tabular}{p{{0.34\columnwidth}}  p{{0.4\columnwidth}} p{{0.215\columnwidth}} c}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Program sources}} & \multicolumn{1}{c}{\textbf{Repository links}} & \multicolumn{1}{c}{\textbf{Primary studies}} & \multicolumn{1}{c}{\textbf{\#}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}  
    MQT bench~\cite{quetschlich2023mqt} & {\footnotesize \url{https://www.cda.cit.tum.de/mqtbench/}} & \cite{\PaperThirtyNine ,\PaperFiftyFour ,\PaperSeventyEight ,\PaperOneHundredAndTwelve} & 4 \\ 
    Bugs4Q~\cite{zhao2021bugs4q} & {\footnotesize \url{https://github.com/Z-928/Bugs4Q}} & \cite{\PaperFortyFour ,\PaperEightyThree ,\PaperEightyFour ,\PaperOneHundredAndNine} & 4 \\ 
    Qbugs~\cite{campos2021qbugs} & N/A & \cite{\PaperFortyFour ,\PaperEightyThree ,\PaperEightyFour} & 3 \\ 
    VeriQBench~\cite{chen2022VeriQBench} & N/A & \cite{\PaperSix ,\PaperFiftyTwo} & 2 \\ 
    O'reilly~\cite{johnston2019programming} & {\footnotesize \url{https://oreilly-qc.github.io/}} & \cite{\PaperTwentySeven ,\PaperFiftyNine} & 2 \\ 
    Qiskit aqua library & {\footnotesize \url{https://github.com/qiskit-community/qiskit-aqua#migration-guide}} & \cite{\PaperSeventyFour ,\PaperOneHundredAndNine} & 2 \\ 
    RevLib~\cite{wille2008revlib} & {\footnotesize \url{https://www.revlib.org/}} & \cite{\PaperFifteen} & 1 \\ 
    Qiskit textbook & {\footnotesize \url{https://qiskit.org/textbook/ch-algorithms/shor.html}} & \cite{\PaperTwentySeven} & 1 \\ 
    Rieffel et al.~\cite{rieffel2011quantum} & N/A & \cite{\PaperFortyThree} & 1 \\ 
    Qiskit circuit library & {\footnotesize \url{https://github.com/Qiskit/qiskit/tree/stable/1.2/qiskit/circuit/library}} & \cite{\PaperFortySix} & 1 \\ 
    Quanto~\cite{pointing2024optimizing} & N/A & \cite{\PaperSeventy} & 1 \\ 
    Juan Carlos et al.~\cite{garcia2011equivalent} & N/A & \cite{\PaperSeventy} & 1 \\ 
    Quantum algorithm zoo & {\footnotesize \url{https://quantumalgorithmzoo.org/}} & \cite{\PaperSeventyThree} & 1 \\ 
    Quantum code repository & {\footnotesize \url{https://quantumcomputinguk.org/code-repository}} & \cite{\PaperSeventyThree} & 1 \\ 
    QASMBench~\cite{li2023qasmbench} & {\footnotesize \url{https://github.com/pnnl/QASMBench}} & \cite{\PaperEightyFour} & 1 \\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq1_learning_models_names.tex <==

\begin{tabular}{p{0.7\columnwidth}  p{0.2\columnwidth} c}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Quantum learning-based models}} & \multicolumn{1}{c}{\textbf{Primary studies}} & \multicolumn{1}{c}{\textbf{\#}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  
    Quantum Convolutional Neural Network & \cite{\PaperThirtySix ,\PaperOneHundredAndSeven ,\PaperOneHundredAndTwentyThree} & 3 \\ 
    Quantum Circuit Learning & \cite{\PaperThirtySix ,\PaperOneHundredAndSeven} & 2 \\ 
    Circuit-centric Quantum Classfiers & \cite{\PaperThirtySix ,\PaperOneHundredAndSeven} & 2 \\ 
    Quantum Distributed Learning Software & \cite{\PaperEightyOne} & 1 \\ 
    Hierarchical Circuit Quantum Classifier & \cite{\PaperOneHundredAndSeven} & 1 \\ 
    Hybrid Quantum Neural Network & \cite{\PaperOneHundredAndSeven} & 1 \\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq2_sources_for_variants.tex <==

\begin{tabular}{p{0.32\columnwidth} p{0.32\columnwidth}  p{0.32\columnwidth} c}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Approaches}} & \multicolumn{1}{c}{\textbf{Sources}} & \multicolumn{1}{c}{\textbf{Primary studies}} & \multicolumn{1}{c}{\textbf{\#}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}  
    Real-world bugs & Bugs4Q & \cite{\PaperFortyFive, \PaperFiftyOne, \PaperEightyThree, \PaperOneHundredAndNine} & 4 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    Imperfect models & MNIST & \cite{\PaperThirtySix, \PaperOneHundredAndSeven} & 2 \\ 
     & Fashion-MNIST & \cite{\PaperThirtySix, \PaperOneHundredAndSeven} & 2 \\ 
     & CIFAR10 & \cite{\PaperOneHundredAndSeven} & 1 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    Mutation toolings & QMutPy & \cite{\PaperSix, \PaperNinetyFour, \PaperOneHundredAndNine, \PaperOneHundredAndNineteen} & 4 \\ 
     & Muskit & \cite{\PaperThirtyNine, \PaperOneHundredAndSixteen} & 2 \\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq4_input_type_names.tex <==

\begin{tabular}{p{0.25\columnwidth}  p{0.35\columnwidth} p{0.38\columnwidth} c}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Test input types}} & \multicolumn{1}{c}{\textbf{Input properties}} & \multicolumn{1}{c}{\textbf{Primary studies}} & \multicolumn{1}{c}{\textbf{\#}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}  
    Initial quantum states & Computational basis states & \cite{\PaperOne, \PaperThree, \PaperFive, \PaperTwelve, \PaperSeventeen, \PaperTwenty, \PaperTwentyOne, \PaperTwentyFour, \PaperThirtyEight, \PaperFiftyTwo, \PaperFiftyNine, \PaperSixty, \PaperSixtySeven, \PaperSeventyOne, \PaperEightyThree, \PaperEightyFour, \PaperOneHundredAndSix, \PaperOneHundredAndEight, \PaperOneHundredAndThirteen, \PaperOneHundredAndFifteen, \PaperOneHundredAndSixteen} & 21 \\ 
     & Fully separable states & \cite{\PaperThirteen, \PaperThirtyFive, \PaperFortyFour, \PaperFiftyTwo, \PaperEightySix, \PaperOneHundredAndThree, \PaperOneHundredAndTwentyTwo} & 7 \\ 
     & Default state & \cite{\PaperOneHundredAndEight, \PaperOneHundredAndTwelve, \PaperOneHundredAndSeventeen, \PaperOneHundredAndTwentyOne} & 4 \\ 
     & States prepared by specific circuits & \cite{\PaperSix, \PaperOneHundredAndFive, \PaperOneHundredAndNineteen} & 3 \\ 
     & Mixed states & \cite{\PaperFortySix, \PaperSeventyOne} & 2 \\ 
     & Superposition states & \cite{\PaperSeventyOne, \PaperOneHundredAndEight} & 2 \\ 
     & State vector by a quantum constraint solver & \cite{\PaperFortyFive} & 1 \\ 
     & Pauli eigenstates & \cite{\PaperSeventy} & 1 \\ 
     & Eigenvector of a unitary operation & \cite{\PaperOneHundredAndSeventeen} & 1 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    Classical inputs & Numbers & \cite{\PaperTwelve, \PaperTwentySeven, \PaperFortySix, \PaperSeventyOne, \PaperOneHundredAndEight} & 5 \\ 
     & Images & \cite{\PaperThirtySix, \PaperEightyOne, \PaperOneHundredAndSeven, \PaperOneHundredAndTwentyThree} & 4 \\ 
     & Vectors & \cite{\PaperFourteen, \PaperFortySix, \PaperOneHundredAndTwentyOne} & 3 \\ 
     & Matrices & \cite{\PaperFortyFour, \PaperFortySix} & 2 \\ 
     & Classical arguments for oracle & \cite{\PaperThirtyThree} & 1 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    Measurement operators & Helstrom measurement operators & \cite{\PaperThirtySeven} & 1 \\ 
     & Pauli strings & \cite{\PaperThirtyNine} & 1 \\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq5_oracle_type.tex <==

\begin{tabular}{c  p{0.47\columnwidth} p{0.37\columnwidth} c}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Test oracles}} & \multicolumn{1}{c}{\textbf{Testing protocols}} & \multicolumn{1}{c}{\textbf{Primary studies}} & \multicolumn{1}{c}{\textbf{\#}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}  
    WOO & Original outcome & \cite{\PaperOne, \PaperThree, \PaperFive, \PaperSeventeen, \PaperTwenty, \PaperTwentyOne, \PaperFortyThree, \PaperFiftyNine, \PaperSixty, \PaperSeventyOne, \PaperSeventyThree, \PaperSeventyEight} & 12 \\ 
     & Inverse test & \cite{\PaperSeventyOne, \PaperOneHundredAndSix, \PaperOneHundredAndEight, \PaperOneHundredAndTwelve} & 4 \\ 
     & Swap test & \cite{\PaperFiftyTwo, \PaperOneHundredAndTwelve} & 2 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    OPO & Pearson's chi-squared test & \cite{\PaperFive, \PaperSeventeen, \PaperTwenty, \PaperTwentyOne, \PaperThirtyOne, \PaperFortyThree, \PaperFiftyTwo, \PaperSixty, \PaperSeventyThree, \PaperSeventyEight, \PaperEightyFour, \PaperOneHundredAndTwelve, \PaperOneHundredAndThirteen, \PaperOneHundredAndFourteen, \PaperOneHundredAndSeventeen} & 15 \\ 
     & Wilcoxon signed rank test & \cite{\PaperThree, \PaperFiftyNine} & 2 \\ 
     & Expectation value & \cite{\PaperThirtyNine} & 1 \\ 
     & Mann-Whitney U test & \cite{\PaperFortySix} & 1 \\ 
     & Jensen-Shannon divergence & \cite{\PaperEightyThree} & 1 \\ 
     & G-test & \cite{\PaperOneHundredAndTwelve} & 1 \\ 
     & Multinomial test & \cite{\PaperOneHundredAndTwelve} & 1 \\ 
     & Monte Carlo Pearson's chi-squared test & \cite{\PaperOneHundredAndTwelve} & 1 \\ 
     & Monte Carlo G-test & \cite{\PaperOneHundredAndTwelve} & 1 \\ 
     & Monte Carlo multionmial test & \cite{\PaperOneHundredAndTwelve} & 1 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    PBO & Original outcome & \cite{\PaperTwentyFour, \PaperTwentySeven, \PaperNinetyFour} & 3 \\ 
     & Pearson's chi-squared test & \cite{\PaperTwelve, \PaperThirteen} & 2 \\ 
     & Fisher's exact test & \cite{\PaperThirtyThree, \PaperOneHundredAndNineteen} & 2 \\ 
     & T test & \cite{\PaperThirteen} & 1 \\ 
     & Swap test & \cite{\PaperSeventy} & 1 \\ 
     & Trace-related distance & \cite{\PaperSeventy} & 1 \\ 
     & Holm-Bonferroni correction & \cite{\PaperOneHundredAndNineteen} & 1 \\ 
     & Ancillary qubit & \cite{\PaperOneHundredAndTwentyTwo} & 1 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    DOO & Frequence-based criterion & \cite{\PaperFifteen, \PaperSeventyOne, \PaperSeventyEight} & 3 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    QSO & Quantum fidelity & \cite{\PaperOneHundredAndFourteen, \PaperOneHundredAndFifteen, \PaperOneHundredAndSeventeen} & 3 \\ 
     & Quantum state tomography & \cite{\PaperOneHundredAndFourteen, \PaperOneHundredAndSeventeen} & 2 \\ 
     & Original outcome & \cite{\PaperOneHundredAndTwelve} & 1 \\ 
     & Bloch vector representation & \cite{\PaperOneHundredAndFifteen} & 1 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    QOO & Quantum process tomography & \cite{\PaperOneHundredAndFourteen, \PaperOneHundredAndSeventeen} & 2 \\ 
     & Quantum fidelity & \cite{\PaperOneHundredAndFourteen, \PaperOneHundredAndSeventeen} & 2 \\
    \cmidrule(lr){1-4} 
    
    \multicolumn{4}{p{1.2\columnwidth}}{\textbf{Total number 
    of primary studies for each test oracle:} OPO (20), WOO (16), PBO (9), QSO (4), DOO (3), QOO (2)}\\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq5_program_specification.tex <==

\begin{tabular}{p{0.25\columnwidth}  p{0.35\columnwidth} p{0.38\columnwidth} c}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Program specifications}} & \multicolumn{1}{c}{\textbf{Output types}} & \multicolumn{1}{c}{\textbf{Primary studies}} & \multicolumn{1}{c}{\textbf{\#}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}  
    Specified & Probability distribution & \cite{\PaperOne, \PaperThree, \PaperFive, \PaperTwelve, \PaperSeventeen, \PaperTwenty, \PaperTwentyOne, \PaperThirtyOne, \PaperThirtyNine, \PaperFiftyNine, \PaperSixty, \PaperSeventyOne, \PaperSeventyThree, \PaperSeventyEight, \PaperEightyFour, \PaperOneHundredAndFourteen} & 16 \\ 
     & Quantum state & \cite{\PaperFourteen, \PaperThirtyEight, \PaperFortyThree, \PaperFortySix, \PaperSeventyOne, \PaperEightyThree, \PaperOneHundredAndSix, \PaperOneHundredAndEight, \PaperOneHundredAndTwelve, \PaperOneHundredAndFourteen, \PaperOneHundredAndFifteen, \PaperOneHundredAndSeventeen, \PaperOneHundredAndTwentyOne} & 13 \\ 
     & Classical outcome & \cite{\PaperFifteen, \PaperThirtySix, \PaperSeventyOne, \PaperEightyOne, \PaperOneHundredAndSix, \PaperOneHundredAndSeven, \PaperOneHundredAndEight} & 7 \\ 
     & Quantum operator & \cite{\PaperThirtySeven, \PaperEightyThree, \PaperOneHundredAndFourteen, \PaperOneHundredAndSeventeen} & 4 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    Derived & General property & \cite{\PaperThirtyThree, \PaperFortyOne, \PaperFortyFour, \PaperFiftyFour, \PaperSeventy, \PaperSeventyFour, \PaperNinetyFour, \PaperOneHundredAndNineteen, \PaperOneHundredAndTwentyTwo} & 9 \\ 
     & Original program output & \cite{\PaperSix, \PaperThirteen, \PaperSeventyFour, \PaperOneHundredAndNine, \PaperOneHundredAndSixteen} & 5 \\ 
     & Metamorphic relation & \cite{\PaperTwentyFour, \PaperTwentySeven} & 2 \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
    Implicit & Program error & \cite{\PaperSeventyFour} & 1 \\
    \cmidrule(lr){1-4} 
    
    \multicolumn{4}{p{1.2\columnwidth}}{\textbf{Total number 
    of primary studies for each program specification:} Specified (32), Derived (15), Implicit (1)}\\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq6_metrics_names.tex <==

\begin{tabular}{p{0.14\columnwidth}  p{0.42\columnwidth} p{0.42\columnwidth}}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{SE problems}} & \multicolumn{1}{c}{\textbf{Effectiveness (\#)}} & \multicolumn{1}{c}{\textbf{Cost (\#)}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  
    Software testing & Percentage of failed tests (15),\newline Mutation score (10),\newline Accuracy (6),\newline Precision (5),\newline Recall (5). & Overall execution time (15),\newline Circuit simulation time (2),\newline Number of gates (2),\newline Number of shots (2),\newline Circuit depth (2),\newline Number of iterations (2). \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
Runtime assertion & Success rate in identifying errors (1),\newline Reduction rate for the number of lines (1),\newline F1 score (1),\newline Fidelity of quantum states (1),\newline False positives (1),\newline Success rate of program execution (1). & Number of gates (3),\newline Number of qubits (3),\newline Number of measurement operators (2),\newline Number of shots (1),\newline Overall execution time (1),\newline Circuit depth (1). \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
Fault localization & Localization rate (1),\newline Probability of successfully locating a bug (1),\newline Mutation score (1),\newline Percentage of statements before finding faults (1). & Number of gates (1),\newline QPU execution time (1). \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
Program repair & Repair rate (3),\newline Distance between the repaired and correct programs (1),\newline Approximation accuracy (1),\newline Number of successful runs (1),\newline Number of equivalent patches (1),\newline Error of similarity (1),\newline Error of unitarity (1). & Overall execution time (2),\newline Repair time (1),\newline Number of gates (1),\newline Test generation time (1),\newline Localization time (1). \\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq7_baseline_comparison.tex <==

\begin{tabular}{p{0.5\columnwidth}  p{0.48\columnwidth}}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Statistical tests (\#)}} & \multicolumn{1}{c}{\textbf{Associated statistics (\#)}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2}  
    Mann-Whitney U test (8) & $p$-value (8), Vargha and Delaney's $\hat{A}_{12}$ statistics (7), Magnitude (2) \\ 
    Fisher's exact test (2) & Odds ratio (2), $p$-value (1) \\ 
    Kruskal-Wallis test (1) & $p$-value (1) \\ 
    Spearman's rank correlation test (1) & Spearman rank coefficient (1) \\ 
    Wilcoxon signed-rank test (1) & $p$-value (1), Cliff's $\delta$ (1) \\
    \cmidrule(lr){1-2}
    \multicolumn{2}{p{\columnwidth}}{\textbf{Total number of primary studies:} 9}\\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq7_baseline_names.tex <==

\begin{tabular}{p{0.15\columnwidth}  c  p{0.7\columnwidth}}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{SE problems}} & \multicolumn{1}{c}{\textbf{Categories}} & \multicolumn{1}{c}{\textbf{Baselines (Correspondings primary studies)}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  
    Software testing & SOTA & QuraTest (\cite{\PaperFortyFive, \PaperOneHundredAndFive}), SimBAy (\cite{\PaperThirtySix}), ETO (\cite{\PaperThirtyNine}), Quito (\cite{\PaperFortyFive}), Pure-state test cases (\cite{\PaperFortySix}), Pearson's chi-squared test (\cite{\PaperOneHundredAndTwelve}), QMutPy (\cite{\PaperOneHundredAndThirteen}), Muskit (\cite{\PaperOneHundredAndThirteen}), QSharpCheck (\cite{\PaperOneHundredAndNineteen}) \\ 
     & Adaption & Adaptive random testing (\cite{\PaperFiftyTwo}), Tradifuzz (\cite{\PaperEightySix}) \\ 
     & Adapted & Swap test (\cite{\PaperOneHundredAndTwelve}), Statevector test (\cite{\PaperOneHundredAndTwelve}), G-test (\cite{\PaperOneHundredAndTwelve}), Multinomial test (\cite{\PaperOneHundredAndTwelve}), Monte Carlo Pearson's chi-squared test (\cite{\PaperOneHundredAndTwelve}), Monte Carlo G-test (\cite{\PaperOneHundredAndTwelve}), Monte Carlo multinomial test (\cite{\PaperOneHundredAndTwelve}) \\ 
     & Naive & Random testing (\cite{\PaperFive, \PaperFiftyTwo, \PaperSixty, \PaperOneHundredAndSeven}), Random search (\cite{\PaperSeventeen, \PaperTwenty, \PaperTwentyOne, \PaperFortyThree}), Random state vector generator (\cite{\PaperFortyFive, \PaperOneHundredAndThree}), Random circuit generator (\cite{\PaperSix}), Random coherent noise (\cite{\PaperThirtySix}), SAMPLE (\cite{\PaperThirtyEight}), Random quantum circuit generator (\cite{\PaperFortyFive}), Noise prediction model based on linear regression (\cite{\PaperSixtySeven}) \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    Runtime assertion & SOTA & QECA (\cite{\PaperFourteen, \PaperOneHundredAndTwentyOne}), Stat (\cite{\PaperFourteen}), Proq (\cite{\PaperOneHundredAndFifteen}) \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    Fault localization & Adaption & Spectrum-based fault localization (\cite{\PaperOneHundredAndNine}) \\ 
     & Naive & Naive linear search (\cite{\PaperThirtyOne, \PaperEightyFour}), Naive binary search (\cite{\PaperThirtyOne, \PaperEightyFour}) \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    Program repair & SOTA & LLM-QAPR (\cite{\PaperFortyFour}) \\ 
     & Adaption & GenProg (\cite{\PaperEightyThree}), TBar (\cite{\PaperEightyThree}) \\     & Composite & Syn-QFST (\cite{\PaperFortyFour}), Syn-QSD (\cite{\PaperFortyFour}), Quito (\cite{\PaperFortyFour}), QuSBT (\cite{\PaperFortyFour}) \\     & Naive & Basic-QAPR (\cite{\PaperFortyFour}) \\
    \cmidrule(lr){1-3}
\multicolumn{3}{p{\columnwidth}}{\textbf{Number of deduplicated baselines:} \newline
    Software testing (26): SOTA (9), Adaption (2), Adapted (7), Naive (8)\newline
    Runtime assertion (3): SOTA (3)\newline
    Fault localization (3): Adaption (1), Naive (2)\newline
    Program repair (8): SOTA (1), Adaption (2), Composite (4), Naive (1)}\\
    \bottomrule[1pt]
\end{tabular}
        

==> figures/generated/rq8_varied_and_adaptive_shots.tex <==

\begin{tabular}{p{0.13\columnwidth}  p{0.68\columnwidth} p{0.20\columnwidth}}
    \toprule[1pt]
    \multicolumn{1}{c}{\textbf{Categories}} & \multicolumn{1}{c}{\textbf{Configuration schemes}} & \multicolumn{1}{c}{\textbf{Primary studies}} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  
    Adaptive & The number of possible outputs for a specific input multiplied by 100 & \cite{\PaperFive, \PaperSeventeen, \PaperTwenty, \PaperTwentyOne, \PaperFiftyTwo} \\ 
     & Configured as $10^4$ for programs with 4 or 5 qubits and $10^5$ for programs with 6 or 7 qubits & \cite{\PaperSix} \\ 
     & Calculated by the selected algorithms and also associated with the testing scenarios & \cite{\PaperThirtyEight} \\ 
     & The rank of program specification multipled by 10 & \cite{\PaperFortyThree} \\ 
     & The minimum shots determined by an estimated lower bound & \cite{\PaperSeventy} \\ 
     & The minimum determined by statistics of Pearson's chi-squared test and increased by 100 per step up to 100000 in accordance with the early determination & \cite{\PaperEightyFour} \\ 
     & The maximum shots determined by the Quantum Chernoff bound & \cite{\PaperOneHundredAndTwelve} \\ 
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
    Varied & From $10^1$ to $10^5$ & \cite{\PaperThirtySix} \\ 
     & From $2^3$ to $2^{10}$ & \cite{\PaperFortySix} \\     & Proportional to the lower bound ranging from 0.05 to 1.0 & \cite{\PaperSeventy} \\     & From $10^0$ to $10^3$ & \cite{\PaperOneHundredAndSix} \\     & From $10^2$ to $10^5$ & \cite{\PaperOneHundredAndSeven} \\     & From $10^0$ to $10^4$ & \cite{\PaperOneHundredAndTwelve} \\     & From $10^0$ to $10^5$ & \cite{\PaperOneHundredAndSeventeen} \\     & From 12 to 3200 & \cite{\PaperOneHundredAndNineteen} \\
    \bottomrule[1pt]
\end{tabular}
        

==> sections_minor_revision/results.tex <==
Zooming into the primary studies, we present the review results and perform a detailed analysis on the basis of the data extraction items collected and annotated by the authors.


\subsection{\RQSection{8}}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/generated/rq8_shot_config_types.pdf}
        \caption{Setting types for shots}  
        \label{fig: rq8_shot_config_types}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/generated/rq8_fixed_shots.pdf}
        \caption{Number of fixed shots}  
        \label{fig: rq8_number_of_repetitions}
    \end{subfigure}

    \begin{subfigure}[b]{0.98\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/generated/rq8_number_of_repetitions.pdf}
        \caption{Histogram for individual repetitions \mq{better to replace infinite with the maximum number}}  
        \label{fig: rq8_number_of_repetitions}
    \end{subfigure}
    \caption{Visualization for shots and repetitions adopted in the primary studies}  
    \label{fig: rq8}
\end{figure}



\begin{table}[!t]
    \footnotesize
    \centering
    \caption{Specific configurations of adaptive and varied shots}
    \label{tab: rq8_varied_and_adaptive_shots}
    \resizebox{.98\columnwidth}{!}{
        \input{tables/generated/rq8_varied_and_adaptive_shots}
    }
\end{table}

TODO
\AnswerToRQ{8}{TODO}
\subsection{\RQSection{9}}


\yc{Numbers instead of prop.}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/generated/rq9_backend_temporal_trend.pdf}
        \caption{Proportion of each backend over years}  
        \label{fig: rq9_backend_temporal_trend}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/generated/rq9_number_of_backends.pdf}
        \caption{Upset plot about the adoption of each backend}  
        \label{fig: rq9_number_of_backends}
    \end{subfigure}

    \begin{subfigure}[b]{0.98\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/generated/rq9_backend_output.pdf}
        \caption{The distribution of output types directly yielded by the ideal simulator, where one study might consider more than one output type}  
        \label{fig: rq9_backend_output}
    \end{subfigure}
    \caption{Backends adopted in the primary studies to run the tested circuits}  
    \label{fig: rq9}
\end{figure}



TODO
\AnswerToRQ{9}{TODO}
\subsection{\RQSection{10}}

\begin{table}[!t]
    \footnotesize
    \centering
    \caption{Available sources of object programs mentioned in the primary studies}
    \label{tab: rq10_available_program_sources}
    \resizebox{.98\columnwidth}{!}{
        \input{tables/generated/rq10_available_program_sources}
    }
    {\justify
        {\fontsize{8pt}{7.5pt}\selectfont
            ``N/A'' indicates the source did not provide an available repository link, but the programs can still be acquired through the literature.
        }
    \par}
\end{table}

\begin{table}[!t]
    \footnotesize
    \centering
    \caption{Available artifacts (up to~\SnowballingEndTime) provided by the primary studies}
    \label{tab: rq10_available_artifacts}
    \resizebox{.98\columnwidth}{!}{
        \input{tables/generated/rq10_available_artifacts}
    }
\end{table}

TODO
\AnswerToRQ{10}{TODO}


==> tables/manual/preliminary_gate_example.tex <==

  \begin{tabular}{l c c}
      \toprule
      Gate & Symbol & Matrix \\
      \midrule

      Pauli-X &
      $\Qcircuit @C=1em @R=.7em {
        & \gate{X} & \qw
      }$ &
      $\begin{bmatrix}
        0 & 1 \\
        1 & 0
      \end{bmatrix}$ \\[0.6em]

      Hadamard &
      $\Qcircuit @C=1em @R=.7em {
        & \gate{H} & \qw
      }$ &
      $\frac{1}{\sqrt{2}}
      \begin{bmatrix}
        1 & 1 \\
        1 & -1
      \end{bmatrix}$ \\[0.6em]

      Rotation-X &
      $\Qcircuit @C=1em @R=.7em {
        & \gate{R_x(\theta)} & \qw
      }$ &
      $\begin{bmatrix}
        \cos(\theta/2) & -i\sin(\theta/2) \\
        -i\sin(\theta/2) & \cos(\theta/2)
      \end{bmatrix}$ \\[0.6em]

      CNOT &
      $\Qcircuit @C=1em @R=.7em {
        & \ctrl{1} & \qw \\
        & \targ    & \qw
      }$ &
      $\begin{bmatrix}
        1 & 0 & 0 & 0 \\
        0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 1 \\
        0 & 0 & 1 & 0
      \end{bmatrix}$ \\

      \bottomrule
    \end{tabular}%

